Using the Buffer to Avoid Rebuffers: Evidence from a Large Video Streaming Service

To provide a better streaming experience, video clients today select their video rates by observing and estimating the available capacity. Recent work has shown that capacity estimation is fraught with difficulties because of complex interactions between the ABR control loop, HTTP server performance and TCP congestion control. Estimation-based rate selection algorithms can lead to unnecessary rebuffering events and suboptimal video quality. This paper argues that we should do away with estimating network capacity, and instead directly observe and control the playback buffer--which is the state variable we are most interested in controlling. We present a class of "buffer-based" rate selection algorithms that reduce the rebuffering rate while allowing us to control the delivered video quality. We implemented our algorithms inside the Netflix video client and ran a series of experiments spanning millions of Netflix users around the world. Our results show that by doing away with estimating network capacity and instead focusing on buffer occupancy, we can reduce rebuffer rates by 20% while holding video rate constant.

==> design.tex <==
\section{The Design Elements of Buffer-Based Algorithms}
\label{sec:design_element}

%Outline:
% -- Background on HTTP Video Streaming: to set the stage
% -- Chunk Map: Explain why rate map is not enough and to motivate chunk map
% -- Describe design principle based on chunk map to achieve the two goals 
% -- Describe how to calculate reservoir size in order to provide zero unnecessary rebuffer guarantee
% -- Describe how to handle temporal network outage by having outage protection

\subsection{Background on HTTP Streaming}
To set the stage, we start with some background on HTTP-based video streaming.
%the video
%rate selection problem in the domain of HTTP-based video streaming.

{\bf Video rates and video chunks}.  For a typical commercial HTTP-based video
streaming service, videos are pre-encoded into a discrete set of
video rates (e.g. 235kb/s, 500kb/s, 1.5Mb/s and so on) and stored as separate files by the CDNs.  When a customer
streams a video, the video client downloads the video piece by piece
by issuing HTTP byte-range requests. The individual pieces are
called {\em chunks}.  A client can only
change its selected video rate on a chunk-by-chunk basis (since this
is the granularity of requests).  Regardless of the encoded video
rate, each video chunk contains the same length of video in seconds of
playback. We denote the video length in each chunk as $V$ seconds. 

For the ease of describing the algorithm, 
in the following we assume the video client can choose from a set
of $m$ discrete video rates, $\{ R_1, \ldots, R_m \}$, where $R_1 <
R_2 < ... < R_{m}$.  We also refer to $R_1$ as
$R_{\min}$ (the minimum video rate), and $R_m$ as $R_{\max}$ (the maximum
video rate).

{\bf The streaming buffer}.  
The streaming buffer in the video client is typically measured in seconds of
playback time.\footnote{This is typical of streaming clients, e.g.,
Silverlight.}  At any time the buffer may contain chunks with many
different video rates, and the output bitrate of the buffer will
depend on the video rate of the chunk currently being played.  As a
result, there is no direct mapping between buffer occupancy in bytes
and buffer occupancy in seconds.  By measuring the buffer in the time
domain, the client keeps a record of how many ``video seconds'' worth
of playback video currently resides in the buffer, without having to
track the video rate associated with each video chunk.  Since the
viewer ultimately cares about playback, streaming clients commonly 
measure the buffer in seconds rather than bytes. Previous literature 
on HTTP video streaming also uses the time-based buffer 
model~\cite{huang12imc:videorate, Tian12conext:buffervideorate}. We let $B_{\max}$ denote 
the buffer capacity in seconds.

{\bf Buffer dynamics.}  
To understand the relationshop how buffer implicitly capture the capacity in term of occupancy, 
here we describe the buffer dynamics in terms of video rate and available capacity. 
We index time by $t \geq 0$, and let $C(t)$ denote the system capacity
at time $t$.  Here, the system capacity represents the overall 
end-to-end capability of the system, including the capacity of the CDN servers, the video client and
the available bandwidth of the network in between. 
We let $B(t)$ be the streaming buffer occupancy at time
$t$ (measured in seconds).  Finally, we let $R(t)$ denote the video
rate selected at time $t$.  
(Note that if the buffer is full, then no chunk can be downloaded at time $t$; thus we
adopt the convention that if $B(t) = B_{\max}$ then $C(t) = 0$.)
Observe that the buffer drains at unit rate (since one second is
played back every second of real time), and fills at rate
$C(t)/R(t)$.  

Given the constraint that we can only select video rates on a
chunk-by-chunk basis, it is useful to consider the buffer dynamics
when observed {\em at the time points when a chunk finishes}.
Let $r[k]$ be the video rate selected for the $k$-th chunk 
and $c[k]$ be the average download capacity for the $k$-th
If each chunk contains $V$ seconds of video, 
the $k$-th chunk is $V r[k]$ bytes long.
Observe that during each chunk download, the buffer drains $V r[k]/c[k]$ seconds while fills with 
$V$ seconds of video.

We summarize the two equivalent models of buffer dynamics in Figure~\ref{fig:buffer_model}.
Note that the above model is simplified, since the most of the encoder in production uses VBR, instead of CBR. 
As a result, the instanteneous video rate might deviate from the video rate $R(t)$, which is the overall average rate. 
However, the above simplified model can help us ration about the relationship between capacity and video rate. 
We will discuss the case of VBR later in the section. 

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{buffer.pdf}
\caption{Two models of the streaming buffer.}
\label{fig:buffer_model}
\end{figure}




\subsection{Rate Map and Design Principles}

\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth]{design_space_general.pdf}
\caption{The design space of rate maps and chunk maps.}
\label{fig:design_space}
\end{figure}

%\begin{figure}[t]
%\centering
%\subfigure[The design space of rate maps.]{\includegraphics[width=0.7\linewidth]{design_space.pdf}\label{fig:design_space_ratemap}}
%\subfigure[The design space of chunk maps.]{\includegraphics[width=0.7\linewidth]{design_space_chunkmap.pdf}\label{fig:design_space_chunkmap}}
%\caption{The design space of buffer-based algorithms.}
%\label{fig:design_space}
%\end{figure}


We first define the design space for Buffer-Based algorithm.
Intuitively, since we select a video rate based solely on the buffer occupancy,
the design space for our algorithms can be expressed as the
buffer-rate plane shown in Figure~\ref{fig:design_space}.  The shaded region
between $[0, B_{\max}]$ on the buffer-axis and $[R_{\min}, R_{\max}]$
on the rate-axis defines the feasible region.  Any curve $f(B)$ on the
plane within the feasible region defines a {\em rate map}, that maps a
current buffer occupancy to a  video rate between $R_{\min}$ and $R_{\max}$.

In~\cite{bufferbased_fhmn}, we have described the design principles to provide guarantees on 
(1) no unnecessary rebuffering and (2) average video rate maximization in an ideal setting. 
We now summarize the principles in the following:

{\bf No unnecessary rebuffering:} As long as $C(t) > R_{\min}$ for all $t$ and we adapt $f(B) \to R_{\min}$ as $B \to 0$, 
we will never unnecessary rebuffering since buffer will start to grow before it is emptied.

{\bf Average video rate maximization:} As long as $f(B)$ is (1) increasing and (2) eventually reaches $R_{\max}$, 
the average video rate will equal to the average capacity when $R_{\min} < C(t) < R_{\max}$ for all $t > 0$. 

In reality, it might be too late to step down to $R_{\min}$ when the buffer is almost empty. 
This is because most video streaming services today use variable bitrate (VBR) in their video encoding, 
and in VBR, when a video encoded at a video rate, the encoder only ensure the {\em average} video rate to be the encoded video rate, while the instantenous video rate varies. 
Figure~\ref{fig:vbrexample} shows the instantaneous video rate over time for a video encoded at 3Mb/s,
where the black line represents the average video rate over all.
Since the video is encoded at 3Mb/s, the encoder ensures the average rate be maintained at 3Mb/s.
As we can see from the figure, the variation on instantaneous video rate can be huge within a video.
Thus, even if the available capacity exactly equals to $R_{\min}$, we will need some buffer to cope with the buffer variation caused by VBR. 
As a result, we will need to right shift the curve $f(B)$ and allocate part of the buffer to absorb the buffer variation at $R_{\min}$. 
We define the amount the curve is right shifted as {\em reservoir} and the buffer operation zone of the curve as {\em cushion}. 
We summarize the updated design principles in Figure~\ref{fig:design_principle}.

\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{vbr_timeseries.pdf}
\caption{The instantaneous video rate of a video encoded at an average rate of 3Mb/s.}
\label{fig:vbrexample}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{design_principle_ratemap.pdf}
\caption{Design Principles coping with VBR.}
\label{fig:design_principle}
\end{figure}

\subsection{Cope with VBR at $R_{\min}$ with Reservoir}
\label{sec:reservoir}

\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{cal_reservoir.pdf}
\caption{Reservoir Calculation.}
\label{fig:reservoir_calc}
\end{figure}

The size of reservoir is the amount of buffer we need to preserve to cope with VBR when capacity is exactly the same as $R_{\min}$.
Since the variation of instantaneous video rate depends on the complexity of scenes, the size of reservoir varies from videos to videos.
As a result, we need to calculate the size of reservoir for each video. 
Figure~\ref{fig:reservoir_calc} shows how the calculation is done. 
When the instantaneous rate is higher than $R_{\min}$, the video client will consume more video in the buffer than the input, since we assume capacity equals to $R_{\min}$.
On the other hand, when the instantaneous rate is lower than $R_{\min}$, the buffer is consumed slower than the input and the buffer occupancy will increase. 
Thus, by summing up the amount of buffer the client will consume minus the amount we can supply during the next $X$ seconds, we can figure out the amount of reservoir we need.

\subsection{Cope with VBR at $R_{2+}$ with Chunk Maps}

Since we should consider the instantaneous video rate in the upcoming video segments, 
it might make more sense to map the buffer occupancy to instantaneous rate, instead of video rate. 
However, since the video is downloaded one chunk at a time, not bit by bit, 
we should map the buffer occupancy to chunk size and figure out which chunk to download from all the available video rates streams.
Thus, we can generalize the design space and make it from the buffer-rate plane to 
the buffer-chunk plane as shown in Figure~\ref{fig:design_space}, 
where the feasible region is defined between $[0, B_{\max}]$ on the buffer-axis and $[Chunk_{\min}, Chunk_{\max}]$ on the chunk-axis, 
where $Chunk_{\min}$ and  $Chunk_{\max}$ represents the minimum and maximum chunk size across all the video rates. 
However, since reservoir has already take care the bitrate variation within the stream of $R_{\min}$, we can safely set $Chunk_{\min}$ as $V R_{\min}$.

\subsection{Video Rate Adaptation Algorithm}

Note that a chunk map by itself does not define an algorithm.  
The chunk size mapped from the chunk map only represents the maximally allowable chunk size according to the buffer occupancy. 
We then figure out the highest possible video rate to request for based on the size of the upcoming chunks in each video rate stream.
Also, since continuously changing the rate might cause the video rate to oscillate.
Instead, we desire an implementation where the video rate is a little ``sticky''.

We therefore use the rate adaptation algorithm described in
Algorithm~\ref{algo:nextRate}. The algorithm follows a
simple principle: it stays at the current video rate as long
as the chuunk size suggested by the chunk map does not pass either the next chunk size from the 
higher available video rate ($\rate_{+}$) or the next lower available
video rate ($\rate_{-}$).
If either of these ``barriers'' are hit, the rate is switched up at most one level at a time 
or down to a new discrete value suggested by the chunk map.
In this way, the buffer distance between the adjacent video 
rates provides a natural cushion to absorb rate oscillations.

\begin{algorithm}
\caption{Video Rate Adaptation Algorithm}
\label{algo:nextRate}
\SetAlgoLined
\KwIn{ $\rate_{\prev}$: The previously used video rate \\ \quad\quad\quad\quad $\buf_{\now}$: The current buffer occupancy  \\ \quad\quad\quad\quad $\chunkmap[\rate]$: The size of the next chunk for each video rate stream }
\KwOut{ $\rate_{\nxt}$: The next video rate }
\BlankLine
\uIf{$\rate_{\prev} = R_{\max}$}{
$\rate_{+} = R_{\max}$
}
\uElse{
$\rate_{+} = \min \{ R_i : R_i > \rate_{\prev} \}$
}

\uIf{$\rate_{\prev} = R_{\min}$}{
$\rate_{-} = R_{\min}$
}
\uElse{
$\rate_{-} = \max \{ R_i : R_i < \rate_{\prev} \}$
}

\uIf{$f(\buf_{\now}) \geq \chunkmap[\rate_{+}] $}{
    $\rate_{\nxt} = \rate_{+}$\;
}
\uElseIf{$f(\buf_{\now}) \leq \chunkmap[\rate_{-}]$}{
    $\rate_{\nxt} = \max \{ R_i : \chunkmap[R_i] < f(\buf_{\now}) \}$\;
}
\uElse{
    $\rate_{\nxt}$ = $\rate_{\prev}$\;
}
\KwRet{$\rate_{\nxt}$}\;
\end{algorithm}

\subsection{Cope with temporal network outage}
By having rebuffer and the chunk map (or rate map), buffer-based algorithm provides the guarantee to not {\em unnecessary} rebuffer. 
Meaning that rebuffer will not happen when the available capacity is equal or larger than $R_{\min}$. 
However, it is not uncommon to have temporal network outage, such as DSL modem retrained. 
A typical temporal network outage can be recovered in $20$ to $30$ seconds. 
To make buffer-based algorithm resilient to temporal network outage, 
we could allocate part of the buffer for outage protection by right shifting the curve. 
By right shifting the curve, the buffer will converge to a higher buffer level for a given available capacity and provide better protection toward temporal network outage. 
We call this portion of buffer literally as ``outage protection''. 
Note that, for ``outage protection'', we can gradually right shifting the curve after the buffer converges to a certain level. 
We do not need to allocate it on the chunk map right at the beginning. 
That is also the reason why we seperate ``outage protection'' from ``reservoir''. 


==> userlevel.tex <==
\section{User Level Analysis}
\label{sec:userlevel}

\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth]{vrate_bba2_norm.pdf}
\caption{The difference on average video rate per user }
\label{fig:userlevel_vrate}
\end{figure}

In the previous sessions, we analyze the performance of the system at the session level. 
However, since the assignment of which algorithm to use happens at the user level, we should also check the performance at the user level. 

First of all, we would like to make sure the buffer-based algorithms significantly improve the rebuffer rate at the user level. 
We performed a Mann–Whitney u-test for the number of rebuffers per playhour per user. 
The analysis shows we have 97-99\% of confidence that the user-level rebuffer rate achieve by the BBA-2 algorithm is lower than the control. 
The only exception is during the off-peak hours, especially between 8am-4pm GMT. During this period, there is no significant difference between BBA-2 and the control.

Second, we run the same u-test for the average video rate per user. 
Despite the analysis we did at the session level shows BBA-2 achieves the same video rate as the control, the user-level analysis shows the BBA-2 achieve lower video rate compare to the control.
Figure~\ref{fig:userlevel_vrate} shows the difference between BBA-2 and control on the average video rate at the account-level throughout the day.
This is because BBA-2 has a closer video rate to the control under more congested network. And people with lower throughput tend to watch more in our system. As a result, the session level result is skewed towards this group of people and makes BBA-2 achieve similar video rate compare to the control at the session level.

